Low-light Environment Neural Surveillance

We design and implement an end-to-end system for real-time crime detection in low-light environments. Unlike Closed-Circuit Television, which performs reactively, the Low-Light Environment Neural Surveillance provides real time crime alerts. The system uses a low-light video feed processed in real-time by an optical-flow network, spatial and temporal networks, and a Support Vector Machine to identify shootings, assaults, and thefts. We create a low-light action-recognition dataset, LENS-4, which will be publicly available. An IoT infrastructure set up via Amazon Web Services interprets messages from the local board hosting the camera for action recognition and parses the results in the cloud to relay messages. The system achieves 71.5% accuracy at 20 FPS. The user interface is a mobile app which allows local authorities to receive notifications and to view a video of the crime scene. Citizens have a public app which enables law enforcement to push crime alerts based on user proximity.

==> maybe_erase.tex <==
\section*{Acknowledgment}
We would like to recognize the guidance provided by Professor Bahram Shafai of Northeastern University, as he gave constant feedback on how to improve the project at each step. We would also like to acknowledge PhD candidate Tim Rupprecht of the Northeastern Computer Vision Lab for early on feedback and guidance on general approaches to deep learning.


\begin{figure}[!h]
    \centering
    \includegraphics[width=6cm]{images/iotarch.JPG}
    \caption{LENS IoT architecture}
    \label{fig:iotarch}
\end{figure}

% NOTE: Is this actually our flow diagram or is it just a graphic that Kevin and Noah pulled from the internet? Just want to make sure it's our stuff.
\begin{figure}[!h]
    \centering
    \includegraphics[width=6cm]{images/awsdiagram.png}
    \caption{AWS service diagram}
    \label{fig:awsdiagram}
\end{figure}

==> supplmental2.0.tex <==
\raggedbottom
\section{LENS Supplemental Material}

% The paper headers



\subsection{SVM improvements}
    \begin{table}[!h]
        \centering
        \addtolength{\leftskip}{-3.5cm}
        \addtolength{\rightskip}{-3.5cm}
        \begin{tabular}{@{}lllll@{}}
        
        \textbf{} &
        \textbf{Theft} & 
        \textbf{Assault} & 
        \textbf{Shooting} &
        \textbf{No Action} \\
        Spatial  & 8 & -48 & 64 & -20 \\
        Temporal & 13 & $\infty$ & 0 & -15 \\
    
        \end{tabular}
        \caption{\label{tab:percentchanges}Percent Changes of spatial stream and temporal stream to SVM fusion}
    \end{table}


